Software model refactoring based on performance analysis: better working on software or performance side?

Several approaches have been introduced in the last few years to tackle the problem of interpreting model-based performance analysis results and translating them into architectural feedback. Typically the interpretation can take place by browsing either the software model or the performance model. In this paper, we compare two approaches that we have recently introduced for this goal: one based on the detection and solution of performance antipatterns, and another one based on bidirectional model transformations between software and performance models. We apply both approaches to the same example in order to illustrate the differences in the obtained performance results. Thereafter, we raise the level of abstraction and we discuss the pros and cons of working on the software side and on the performance side.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v{n}: \\
Formal Engineering Approaches to Software Components \\
and Architectures 2013 (FESCA'13)\\
EPTCS 108, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.108.3}{10.4204/EPTCS.108.3}}
\pdfoutput=1

